Clinically Plausible Pathology-Anatomy Disentanglement in Patient Brain MRI with Structured Variational Priors

We propose a hierarchically structured variational inference model for accurately disentangling observable evidence of disease (e.g. brain lesions or atrophy) from subject-specific anatomy in brain MRIs. With flexible, partially autoregressive priors, our model (1) addresses the subtle and fine-grained dependencies that typically exist between anatomical and pathological generating factors of an MRI to ensure the clinical validity of generated samples; (2) preserves and disentangles finer pathological details pertaining to a patient's disease state. Additionally, we experiment with an alternative training configuration where we provide supervision to a subset of latent units. It is shown that (1) a partially supervised latent space achieves a higher degree of disentanglement between evidence of disease and subject-specific anatomy; (2) when the prior is formulated with an autoregressive structure, knowledge from the supervision can propagate to the unsupervised latent units, resulting in more informative latent representations capable of modelling anatomy-pathology interdependencies.

==> BlurredLesionsWithArrows.tex <==
\begin{picture}(120, 160)
        \put (0, 78.5) {\includegraphics[clip, trim={23cm 0.3cm 0.4cm 0.3cm}, width=0.3\linewidth]{Visuals/Intro/IntroInputReconstructions.png}}
        \put (65, 78.5) {\includegraphics[clip, trim={23cm 0.3cm 0.4cm 0.3cm}, width=0.3\linewidth]{Visuals/Intro/IntroLesions.png}}
        \put(0, 0) {\includegraphics[clip, trim={15.4cm 0.3cm 8cm 0.3cm}, width=0.3\linewidth]{Visuals/Intro/IntroInputReconstructions.png}}
        \put (65,0) {\includegraphics[clip, trim={15.4cm 0.3cm 8cm 0.3cm}, width=0.3\linewidth]{Visuals/Intro/IntroLesions.png}}
        \put(-53,160){\tiny Sampled}
        \put(7,160){\tiny Reconstructed}
        \put(68,160){\tiny Predicted Lesions}
        \put(9,129){\thicklines\color{yellow}\vector(2,1){12}}
        \put(9,50){\thicklines\color{yellow}\vector(2,1){12}}
        \put(5,105){\thicklines\color{yellow}\vector(2,1){12}}
        \put(5,25){\thicklines\color{yellow}\vector(2,1){12}}
        \put(-19,108){\thicklines\color{red}\vector(-2,1){12}}
        \put(-78,95){\rotatebox{90}{\tiny \textsc{Mean-Field}}}
        \put(-78,20){\rotatebox{90}{\tiny \textsc{Structured}}}
        % \put(0, 59){\linethickness{1.5pt}\color{white}\line(1,0){120}}
      \end{picture}

==> InvalidLesions.tex <==
\begin{picture}(60, 160)\label{fig:IntroImpossibleMSLesions}%
\put (0, 78) {\includegraphics[clip, trim={0.2cm 0 0.2cm 0}, width=0.3\linewidth]{Visuals/Intro/InvalidLesion0.png} } 
\put (0, 0) {\includegraphics[clip, trim={0.3cm 0.2cm 0.3cm 0.2cm}, width=0.3\linewidth]{Visuals/Intro/ProperLesion2.png}}
\end{picture}

==> StyleMixing.tex <==
       \begin{picture}(100, 220)
       \hspace{-5.0em}
       \put (0, 150){\includegraphics[width=0.45\linewidth]{Visuals/ADNIOriginal.png}}
       \put (100, 150){\includegraphics[width=0.535\linewidth]{Visuals/BRAVOOriginal.png}}
       \put (5, 215){\tiny Brain MRIs of AD patients}
       \put (20, 215){\tiny  }
       \put (110, 215){\tiny Brain MRIs of MS patients}
       \put (100,-1.5){\includegraphics[trim={0cm 0cm 0cm 0cm}, width=0.535\linewidth]{Visuals/StyleMixingQuadrantsBRAVO.png}}
       \put (0, -1.5) {\includegraphics[trim={0cm 0cm 0cm 0cm}, width=0.45\linewidth]{Visuals/StyleMixingQuadrantsADNI.png}}
       \put (18,147) {\tiny A1 \quad \quad \quad \quad \quad  A2}
       \put (18,136) {\tiny A1 \quad \quad \quad \quad \quad  A2}
       \put (7,130) {\tiny pathology \quad \quad pathology}
       \put (123,147) {\tiny B1 \quad \; \quad \quad \quad \quad \quad B2}
       \put (123,136) {\tiny B1 \quad \; \quad \quad \quad \quad \quad B2}
       \put (110,130){\tiny pathology \; \quad \quad \quad pathology}
       % \put(92,30){\rotatebox{90}{\tiny B2 \quad \quad \quad  \quad \quad  \quad  B1}}
       \put(97,12){\rotatebox{90}{\tiny B2 anatomy \quad \quad  \quad  B1 anatomy}}
       \put(-4,12){\rotatebox{90}{\tiny A2 anatomy \quad \quad \quad A1 anatomy}}
       % \put(0,30){\rotatebox{90}{\tiny A2 \quad \quad \quad  \quad \quad  \quad  A1}}
      \end{picture}
